Types for Location and Data Security in Cloud Environments

Cloud service providers are often trusted to be genuine, the damage caused by being discovered to be attacking their own customers outweighs any benefits such attacks could reap. On the other hand, it is expected that some cloud service users may be actively malicious. In such an open system, each location may run code which has been developed independently of other locations (and which may be secret). In this paper, we present a typed language which ensures that the access restrictions put on data on a particular device will be observed by all other devices running typed code. Untyped, compromised devices can still interact with typed devices without being able to violate the policies, except in the case when a policy directly places trust in untyped locations. Importantly, our type system does not need a middleware layer or all users to register with a preexisting PKI, and it allows for devices to dynamically create new identities. The confidentiality property guaranteed by the language is defined for any kind of intruder: we consider labeled bisimilarity i.e. an attacker cannot distinguish two scenarios that differ by the change of a protected value. This shows our main result that, for a device that runs well typed code and only places trust in other well typed devices, programming errors cannot cause a data leakage.

==> typeRules.tex <==
% !TEX root = main.tex

\subsection*{Other Type Rules for Commands}




%We provide a way to dynamically compare the confidentiality of two rights: 
%This is useful since a device may have assigned the same keys to different names and therefore a right may be more confidential or not depending on the run.

\begin{gather}
\inferrule{
 \vprin \cup \{ R_2 \subseteq R_1\} ; \pc; \Gamma \vdash C_1  
\\ \vprin;\pc;\Gamma \vdash C_2 
}{ \vprin;\pc;\Gamma \vdash \compare{R_1}{R_2}{C_1}{C_2}} 
\tag{compare\_T} \label{type:compare}
\end{gather}



\begin{gather}
\inferrule{
   S \neq \pubKeyType \\ 
   \typeVar{e : S_{R_2}} \\
   \vprin \vdash R_1 \subseteq \pc \cap R_2 \\
  \vprin;\pc;\Gamma \vdash C 
}{
\vprin;\pc;\Gamma \vdash  \assign{x}{e}; ~C } \tag{assign\_T}\label{type:assign}
% \end{gather}
\\ 
% \begin{gather}
\inferrule{
     \typeVar{e_1:\Int_{R_1}} \\
     \typeVar{e_2 : S_{R_2}} \\
     \typeVar{x : \arrayType{S}_{R_3}} \\
    S \neq \pubKeyType \\
   \vprin \vdash R_3 \subseteq \pc \cap R_1 \cap R_2 \\
  \vprin;\pc;\Gamma \vdash C 
}{
\vprin;\pc;\Gamma \vdash  \assign{x[e_1]}{e_2}; ~C } \tag{assign\_array\_T}\label{type:assignArray}
%\end{gather}
\\
%\begin{gather}
\inferrule{ \typeVar{v_1\!:\!B_R} \dots  \typeVar{v_n\!:\!B_R}}{
\typeVar{ \{v_1, \dots v_n \} : \arrayType{B}_R}}
\tag{array\_T} \label{type:array} 
\\[0.4cm]
\inferrule{ \typeVar{x\!:\! \arrayType{B}_{R_1}} \\ e:Int_{R_2} \\ R \subseteq R_1 \cap R_2 }{
\typeVar{ x[e]\!:\!B_R}}
\tag{element\_T} \label{type:element} 
\end{gather}

\begin{gather}
\inferrule{ 
   \typeVar{e_1 : S_{R_1}} \\
   \typeVar{e_2 : S_{R_2}} \\
   \vprin;\pc \cap R_1 \cap R_2; \Gamma \vdash C_1 \\
  \vprin;\pc \cap R_1 \cap R_2; \Gamma \vdash C_2 
}{ \vprin;\pc;\Gamma \vdash \cond{e_1}{e_2}{C_1}{ C_2}} \tag{if\_T}\label{type:if}
\end{gather}
%
%
%\begin{gather}
%\inferrule{ 
%\typeVar{P} : \prinType \\
%\typeVar{k} :  \pubKeyType_{\bot} \\
%\vprin \vdash  \{P,k\} \subseteq R \subseteq \pc   \\
%\vprin;\pc \cap R;\Gamma \cup \{ c : \chanType{S_R}\} \vdash C 
%}{\vprin;\pc;\Gamma \vdash \connectCCert{c}{S_R}{k}{P} ;~ C }
%\tag{connect\_2\_T}\label{type:open-cert-client}
%\end{gather}


\begin{gather}
\inferrule{
\vprin;\pc;\Gamma \vdash G \{C / \nop \}   
}{
\vprin;\pc;\Gamma \vdash \sync\{G\};C }  
\tag{sync\_T} \label{type:sync}
\end{gather}
Where 
\[
\begin{array}{rcl}
G & ::= & \cond{e_1}{e_2}{G_1}{G_2} \\
& | & \new{x}{S_R}{e};~G  \\
& | & \assign{x}{e};~G \\
& | & \assign{x[e_1]}{e_2};~G\\
& | & \compare{R_1}{R_2}{G_1}{G_2}\\
& | & \decrypt{P}{e}{x}{S_R}{G_1}{G_2} \\
& | & \register{P_1}{e}{P_2}{G_1}{G_2} \\
& | & \nop 
\end{array}
\]
%e.g. only use commands which does not imply communications or parallel composition. 


%We define $C_1;skip$ to match any commands ending in a skip.




\begin{gather}
\inferrule{
\vprin;\pc;\Gamma \vdash C_1 \\
\vprin;\pc;\Gamma \vdash C_2
}{
\vprin;\pc;\Gamma \vdash ~C_1~|~C_2 }  
\tag{bang\_T} \label{type:bang}
%\end{gather}
\\
%\begin{gather}
\inferrule{
}{
\vprin;\pc;\Gamma \vdash \nop }  
\tag{skip\_T} \label{type:skip}
%\end{gather}
\\
%\begin{gather}
\inferrule{\vprin;\pc;\Gamma \vdash C
}{
\vprin;\pc;\Gamma \vdash ~\bang C }  
\tag{para\_T} \label{type:paral}
\end{gather}


\subsection*{Other Semantic Rules}

%At run time (unlike when type checking) the set of rights will be instantiated public keys, therefore subset on rights can be checked directly. 

%so the subset  

\begin{gather}
 \inferrule{
  M(R_1) \subseteq M(R_2)
 }{ 
 \dev{M}{\compare{R_1}{R_2}{C_1}{C_2}}
 \rightarrow \dev{M}{C_1}}
 \tag{compare1\_S} \label{red:compare1}
 \end{gather}

 \begin{gather}
 \inferrule{
  M(R_1) \not\subseteq M(R_2)
 }{ 
 \dev{M}{\compare{R_1}{R_2}{ C_1}{C_2}}
 \rightarrow \dev{M}{C_2} 
 }\tag{compare2\_S} \label{red:compare2}
\end{gather}






\begin{gather}
\inferrule{ 
   \dev{M}{C_1}  \rightarrow^*  \dev{M'}{\nop}
 }{
   \dev{M}{ \sync\{C_1\};C_2 }  \rightarrow  \dev{M'}{C_2}
}
 \tag{sync\_S}  \label{red:sync}
\end{gather}

%Here  $\rightarrow^*$ means any number of reduction. 
%N.B. $C_1$ must reduce to $\nop$ on its own, i.e., communications with other processes are not allowed. 




\begin{gather}
 \inferrule{
 M((e_1) = v \\
 M(e_1) = v 
 }{
 \dev{M}{\cond{e_1}{e_2}{C_1}{C_2}}
 \rightarrow \dev{M}{C_1} 
 }\tag{if1\_S} \label{red:if1}
 \\
 \inferrule{
 M((e_1) = v' \\
 M(e_1) = v' \\
  v \neq v' 
  }{
 \dev{M}{\cond{e_1}{e_2}{C_1}{C_2}}
 \rightarrow \dev{M}{C_2} 
 }\tag{if2\_S} \label{red:if2}
% \end{gather}
\\
% 
% \begin{gather}
\inferrule{
 \dev{M}{C_1}|\dev{M_2}{C_3} \rightarrow \dev{M'}{C'_1} |\dev{M'_2}{C'_3}
 }{
 \dev{M_1}{\paral{C_1}{C_2}} | \dev{M_2}{C_3}
 \rightarrow \dev{M'}{\paral{C'_1}{C_2}}| \dev{M'_2}{C'_3}
 }\tag{comp\_S} \label{red:paral}
% \end{gather}
\\
% \begin{gather}
 \inferrule{
 }{
 \dev{M}{~ \bang{C} }
 \rightarrow \dev{M}{ C~|~\bang{C}}}\tag{bang\_S} \label{red:bang}
% \end{gather}
\\
% 
% 
% \begin{gather}
 \inferrule{
M(e) = v_2
 }{
 \dev{M\cup\{x \mapsto v_1\}}{\assign{x}{e}; ~C}
 \rightarrow \dev{M \cup \{x \mapsto v_2\}}{C}
 }\tag{assign\_S} \label{red:assign}
\end{gather}



\begin{gather}
 \inferrule{
M(e_1) = i \\
M(e_2) = v
 }{
 \dev{M\cup\{x \mapsto \{v_1,\dots v_i, \dots v_n\}}{\assign{x[e_1]}{e_2}; ~C}
 \\ \rightarrow \dev{M \cup \{x \mapsto  \{v_1,\dots v, \dots v_n\}\}}{C}
 }\tag{assignArray\_S} \label{red:assignArray}
\end{gather}


Plus the standard rules for evaluating sums. 


\subsubsection*{Other Type Rules for Values}




\begin{gather}
\inferrule{ v\!:\!T \in \Gamma}{ \typeVar{v} : T} \tag{var\_T}\label{type:var}
\end{gather}


\begin{gather}
\inferrule{ 
}{ \typeVar{i} : \Int_\bot} \tag{int\_T}\label{type:int}
\end{gather}



\begin{gather}
\inferrule{ \typeVar{P} : \prinType}{ \typeVar{\publicKey{P}} : \pubKeyType_{\bot}} \tag{pubKey\_T}\label{type:pubKey}
\end{gather}

\subsubsection*{Other Semantic Rules for Values}

\begin{gather}
 \inferrule{
 M(e) = i \\
 M(x) = \{v_1,\dots,v_i,\dots,v_n\}
 }{ 
 M(x[e]) = v_i
} \tag{element\_E}\label{red:arrayelement}
\end{gather}

\begin{gather}
 \inferrule{
 M(P) =  \prin{\pubKey}{\secKey}{R} 
 }{ 
 M(\publicKey{P}) = \pubKey
} \tag{pub\_E}\label{red:pub}
\end{gather}


Plus the standard rules for typing sums. 


\subsection{Equivalence rules}

Reduction is defined modulo the standard equivalence rules, which may be applied in any context, e.g.\\

$D_1 ~|~ D_2 \equiv D_2 ~|~ D_1$ \\
$D_1 ~|~ (D_2 ~|~ D_2) \equiv (D_1 ~|~ D_2) ~|~ D_2$ \\
$\dev{M_1}{C_1~|~C_2} \equiv \dev{M_1}{C_2~|~C_1}$ \\
$\dev{M_1}{C_1~|~(C_2~|~C_3)} \equiv \dev{M_1}{(C_1~|~C_2)~|~C_2}$ \\

\subsection{Comparing Rights}

These are the rules used to decide rights inclusion at the compile-time.  
The set $\vprin$ provides a first set of relation for confidentiality.
It is also possible to directly check the relation when both sets a explicitly given.

 \begin{gather}
\inferrule{ 
R_1 \subseteq R_2
}{
\vprin \vdash R_1\subseteq R_2 } 
\tag{straight}\label{type:straight}
\\
\inferrule{
}{  \vprin \vdash R \subseteq \bot} \tag{$\bot$}\label{type:bot}
\\
\inferrule{
\vprin \vdash R_1 \subseteq R_2
\\ \vprin \vdash R'_1 \subseteq R'_2
}{
\vprin \vdash R_1 \cup R'_1 \subseteq R_2 \cup R'_2
} \tag{union}\label{type:union}
\\
\inferrule{ R_1 \subseteq R_2 \in \vprin
}{\vprin \vdash R_1 \subseteq R_2}  \tag{init}\label{type:init-rights}
\\
\inferrule{\vprin\vdash R_1 \subseteq R_2 \quad \vprin \vdash R_2 \subseteq R_3}{\vprin \vdash R_1 \subseteq R_3}  \tag{trans}\label{type:transitivity}
 \end{gather}




==> types-examples.tex <==
\section{Examples}

In this example, we encode a server which can accept a finite set of accounts.
An account is set up for one or two principals and allow them to 
store private data and ask for computations about these data.
Once an account has been created, 
the first member of the account can do three kind of operations to his account:
\begin{itemize}
 \item first, he can upload data (here an integer) into the server.
 \item next, he can ask the server for the result of a computation based on his data.
 \item finally, he can ask to transfer its data to another account whenever the members of the other account
 are a subset of the initial account.
\end{itemize}
While users data are ensured to remain private (only the server and the members can access it),
the server is still able to maintain statistical record about how many operation has been done for each account.

\begin{code}
 Main := \\
 \nwp{Server}{\{\}};\\
 \new{Array(int)}{$\bot$}{usage} \{0,0,0,0,0 \};\\
 \new{int}{$\bot$}{nextId} 0;\\
 \new{int}{$\bot$}{lock}0;\\
 \new{Enc(int)}{$\bot$}{init} $\encrypt{\publicKey{Server}}{\{\publicKey{Server}\}}{0}$;\\
 \new{Enc(int)}{$\bot$}{stores} \{init,init,init,init,init\};\\
 \new{int}{$\bot$}{status} \{0,0,0,0,0\};\\
 $\paral{ \bang{register}}{\bang{stats}}$\\
\end{code}

The register process ensures that each userId is unique. 
For that it uses a lock that prevents two parallel processes to use nextId at the same time.

\begin{code}
 Register := \\
 \opc{c}{PubK,PubK, int};\\
 \new{int}{$\bot$}{userId} 0;\\
 \bang{}\begin{bl}
 lock = lock + 1;\\
 if(lock = 1)
 \begin{bl}
 if(userId = 0)
 \begin{bl}
  userId = nextId;\\
  nextId = nextId + 1 ;\\
  lock = lock - 1 ;\\
  \In{principal,nextPrincipal,v}{c};\\
  \new{int}{\{$\publicKey{Server}$,principal,nextPrincipal\}}{data}0;\\
  \Out{principal,nextPrincipal,userId}{c};\\
  $\paral{\bang{Upload}}{\paral{\bang{Download}}{\paral{\bang{SendToOtherAccount}}{\bang{ReceiveFromOtherAccount}}}}$
 \end{bl}
 else
 \begin{bl}
    lock = lock -1;
 \end{bl}
  \end{bl} 
 else
 \begin{bl}
  lock = lock -1;
 \end{bl}
 \end{bl}

\end{code}

\begin{code}
 Upload := \\
 \oscf{u}{\bot}{int_{\{\publicKey{Server},principal,nextPrincipal\}}}{Server}{principal};\\
 \In{x}{u};\\
 usage[userId]=usage[userId]+1;\\
 data=x;\\
 \\
 Download := \\
 \oscf{d}{\bot}{int_{\{\publicKey{Server},principal,nextPrincipal\}}}{Server}{principal};\\
 usage[userId]=usage[userId]+1;\\
\Out{f(data)}{d}
\end{code}

The two next processes enable the transfer of data from one account to another account:
the first process which is a sub-process of the sending account stores the data encrypted in the store buffer and
warn the process of the other account that it get some data through the status variable.
The second process which is a sub-process of the receiver account checks for notifications about received data and, 
if any, transfers them to the account's data.
\begin{code}
SendToOtherAccount := \\
\opc{t}{int};\\
\In{to}{t};\\
if(status[to]=0)
\begin{bl}
 stores[to]=$\encrypt{\publicKey{Server}}{\{\publicKey{Server},principal,nextPrincipal\}}{data}$;\\
 status[to]=1;\\
 $!$\{if(status[to]=2)
 \begin{bl}
  \Out{0}{t};\\
  stats[to]=0;
 \end{bl}\}
\end{bl}
\end{code}

\begin{code}
ReceiveFromOtherAccount := \\
if(status[userId]=1)
\begin{bl}
 $\decrypt{Server}{stores[userId]}{packet}{int_{\{\publicKey{Server},principal,nextPrincipal\}}}$
 \begin{bl}
  data=packet;\\
  status[userId]=2;
 \end{bl}
 else
 \begin{bl}
  status[userId]=2;
 \end{bl}
\end{bl}
\end{code}

% 
% \subsection{Echo protocol}
% Client side
% 
% \begin{code}
%  \nwp{pAlice}{\{\}};\\
% % \act{sk}\begin{bl}
%   \new{int}{\{pAlice.pub,server\}}{share} 5;\\
%   \occ{server}{pAlice}{c}{int}{\{pAlice.pub,server\}};\\
%   \Out{\var{letter}}{c};\\
%   \In{reception}{c};
%  %\end{bl} 
% \end{code}
%   
% Server side
% 
% \begin{code}
% %\act{server.priv}\begin{bl}
% \load{server};\\
%   \osc{server}{c}{int}{p} ; \\
%   \In{letter}{c}; \\
%   \Out{\var{letter}}{c}; 
% %\end{bl}
% \end{code}
% 
% \subsection{Tansfering from Alice to Bob through Server}
% 
% Alice side (Alice already know pkB, the public key of Bob and pkB, the public key of the server):
% 
% \begin{code}
% \load{pAlice};\\
%  %\nwp{pAlice}{\{\}};\\
% %  \act{pAlice}\begin{bl}
%   \new{int}{\{pAlice.pub,pkB,pkS\}}{share} 5; \\
%  % \new{\ProtectValue(int)}{\{pAlice.pub,pkB,pkS\}}{letter} \protection{\var{share}}{\{pAlice.pub,pkB,(pkS)\}}{\{pAlice.pub,pkB,pkS\}}; \\
%   \occ{pkS}{pAlice}{c}{\Int}{\{pAlice.pub,pkB,pkS\}};\\
%   \Out{\var{letter}}{c};
% % \end{bl}
%  \end{code}
% 
% Bob side:
% 
% \begin{code}
% \load{pBob};\\
% %\nwp{skB,pkB}{\{\}};\\
% % \act{pBob}\begin{bl}
%   \occ{pkS}{pBob}{c}{int}{\{pkA,pBob.pub,pkS\}};\\
%   \In{Letter}{c};\\
%  % \unpack{int}{a1}{letter}{\var{protectedLetter}}{\lab{\{pkA,pBob.pub,(pkS)\}}}\begin{bl}
%   %  \new{int}{\{pkA,pBob.pub,(pkS)\}}{share} \var{letter};
%   %\end{bl}
%    %else\begin{bl}
%     %  skip;\end{bl}
% % \end{bl}
% \end{code}
% 
% Server side:
% 
% \begin{code}
% \load{pServer};\\
% \oscf{pServer}{pAlice}{c1}{\Int}{\{pServer.pub,pkA,pkB\}};\\
%  \In{letter}{c1};\\
% \oscf{pServer}{pBob}{c2}{\Int}{\{pServer.pub,pkA,pkB\}};\\
%  \Out{\var{letter}}{c2}; 
% \end{code}
% 
% \subsection{Transfering from Alice to Bob through encryption}
% Alice side:
% 
% \begin{code}
%  %\nwp{skA,pkA}{\{\}};\\
%  \load{pAlice};\\
%   \new{\Int}{\{pAlice.pub,pkB\}}{letter}  5;\\
%  % \new{\ProtectValue(int)}{\{pAlice.pub,pkB\}}{letter} \protection{\var{share}}{\{pAlice.pub,pkB\}}{pkB};\\
%   \new{\Cipher(\Int)}{bot}{cipherLetter}  \enc{\var{letter}}{\{pAlice.pub,pkB\}};\\
%   \opc{c}{\Cipher(\Int)};\\
%   \Out{\var{cipherLetter}}{c};
% \end{code}
% 
% Bob side:
% 
% \begin{code}
% \load{pBob};\\
% %\nwp{skB,pkB}{\{\}};\\
% %\act{pBob}\begin{bl}
%   \opc{c}{\Cipher(\Int)};\\
%   \In{ciferText}{c};\\
%   \dec{\Int}{\{pBob.pub,pkA\}}{letter}{\var{ciferText}}{pBob})\begin{bl}
%    % \unpack{int}{a1}{letter}{\var{freezeedLetter}}{\lab{\{pkA,pBob.pub\}}}\begin{bl}
%       \new{\Int}{\{pkA,pBob.pub\}}{share} \var{letter};\end{bl}
%     else \begin{bl}
%       skip;\end{bl}
% \end{code}
% 
% \subsection{Transfering from Alice to Bob through a shared identity}
% Alice side:
% 
% \begin{code}
% \load{pAlice};\\
%  %\nwp{skA,pkA}{\{\}};\\
% % \act{pAlice}\begin{bl}
%   \nwp{pShare}{\{pAlice.pub,pkB\}};
%   \begin{bl}
% 	\new{\Cipher(\SecK)}{bot}{encKey} \enc{\var{$\release{pShare}$}}{\{pAlice.pub,pkB\}};\\
% 	\opc{c}{\Cipher(\SecK)};\\
% 	\Out{encKey}{c};\\
% 	\new{\Int}{\{pShare.pub\}}{share} 5;\\
% 	\oscf{pShare}{pShare.pub}{c2}{\Cipher(\Int)}{\{pShare.pub\}};
% 	\Out{share}{c2};
%   \end{bl}
% %  \act{pShare}\begin{bl}
% %     
% %     \new{\Cipher(\Int)}{bot}{cipherText}  \enc{share}{pShare};\\
% %     \opc{pc}{cipher(int)};\\
% %     \Out{cipherText}{c};
% %  \end{bl}
% % \end{bl}
% \end{code}
% 
% Bob side:
% 
% \begin{code}
% \load{pBob};\\
% %\nwp{skB,pkB}{\{\}};\\
% %\act{pBob}\begin{bl}
%   \opc{c}{\Cipher(\SecK)};\\
%   \In{ciferSkey}{c};\\
%   \dec{\SecK}{\{pBob.pub,pkA\}}{skey}{\var{ciferSkey}}{pBob})
%   \begin{bl}
% $	\register{pBob}{skey}{pShared};$\\
% $	\THEN$
% 	\occ{pShared.pub}{pShared}{c2}{\Int}{\{pShare.pub\}};\\
% 	\In{value}{c2};
%   \end{bl}
% 
% \end{code}

% \subsection{Alice sending data to the server}
% 
% \act{pAlice}\begin{bl}
%     \new{int}{\{Alice,Bob\}}{v}=9;\\
%     \ousc{pserver}{c}{int};\\
%     \In{v}{c};
% \end{bl}
% \subsection{An init protocol}
% In this protocol, we consider that we have a client that interact with a list of friends.
% The information about the firends are on a server.
% We want the client to be able to interact with a particular friend or look for a friend corresponding to some criteria. 
% 
% 
% % This protocol is assumed to be done at the start of any program: 
% % the principal key is recovered, then the public key of all principals and finally the data that are shared with these principals.
% % The client has an a priori knowledge that only 3 integers are shared with each friends but does not know how many friends he has. 
% 
% Client
% \begin{code}
%  \load{me};\\
%  \opc{c1}{\PubK};\\
%  \In{pServer}{c1};\\
%  \opc{c2}{\Int}
%  \In{nbFriends}{c2};\\
%  \new{\Int}{$\bot$}{i}1;\\
%  while(i != nbFriends)\begin{bl}
%      \In{Princi[i]}{c1};\\
%        i=i+1; 
%          \end{bl}
% \new{\Int}{*}{name} Name;\\
% \new{\Int}{*}{surname} Surname;\\
% \new{\Int}{*}{status} Unknown;\\
% i=0;\\
%   while(i != nbFriends)\begin{bl}
%   \new{\Int}{$\bot$}{i}1;\\
%   let $\alpha$= \{ me.pub, Princi[i]\} , \{ me.pub, Princi[i], pServer\} ; \\
% \occ{me}{pServer}{cr}{\Int}{$\alpha$}
% 	     \In{x}{cr};\\
% 	     name[i]=;\\
% 	     \In{y}{cr};\\
% 	     $\alpha$.surname=y;\\
% 	     \In{z}{cr};\\
% 	     $\alpha$.status=z;\\
% 	     i=i+1;
% 	     \end{bl}
% \new{\Int}{$\bot$}{j}0;\\
%   while(j != nbFriends)\begin{bl}
%   fork\begin{bl}
% 	\occ{me}{Princi[i]}{cs}{\Int}{$\alpha[j]$};\\
%        \In{active}{cs};\\
%        $\alpha[j]$.status=responding;
%       \end{bl}
% 	     j=j+1;
% 	\end{bl}
% \end{code}



% \subsection{The collect's point protocol}
% In this protocol, the Server is used as an intermediate between a sender and a receiver.
% The sender sends a request to the server to be able to send values to a given sender.
% Then the sender can sends data to the server.
% If the receiver connects to the Server, it receives data only if the sender creates an account for him.
% In case, the sender have not send anything, the receiver receive a default value. 
% 
% Sender i:
% \begin{code}
%  \new{\Int}{\{Sender.pub,pBox,pReceiver\}}{secret} 3 ;\\
%  \occ{pBox}{Sender.pub}{c}{\PubK}{$\bot$};\\
%  \Out{Sender.pub}{c};\\
%  \Out{pReceiver}{c};\\
%  if(secret != 0)\begin{bl}
%  \occ{pBox}{Sender.pub}{c2}{\Int}{\{Sender.pub,pBox,pReceiver\}};\\
%  \Out{secret}{c2};
%  \end{bl}
% \end{code}
% 
% May be the receiver :
% \begin{code}
%  \occ{pBox}{Bob}{c}{\Int}{\{pSender,pBox,Bob.pub\}};\\
%  \In{parcel}{c};
% \end{code}
% 
% 
% 
% The Box store
% \begin{code}
%  \osc{Box}{c}{\PubK}{$\alpha$};\\
%  if( $\alpha \lc \bot$)
%  \begin{bl}
%  \In{sendi}{c};\\
%  \In{receiveri}{c};\\
%  \new{\Int}{\{sendi,receiveri,Box.pub\}}{parceli} 0;\\
%  \dots \\ 
%  \FORK \begin{bl}
%  \osc{Box}{c1}{\Int}{$\alpha_i$};\\
%  \In{parcel}{c1};\\
%  if($\alpha_i \lc $\{sendi,receiveri,Box.pub\} )
%  \begin{bl}
% 	parceli = parcel;
%  \end{bl}
%  \end{bl}
%  \FORK \begin{bl}
%  \osc{Box}{c2}{\Int}{$\beta_i$};\\
%  if(\{sendi,receiveri,Box.pub\}$ \lc \beta_i$)
%  \begin{bl}
%   \Out{parceli}{c2}
%  \end{bl}
% 
%  \end{bl}
%  \end{bl}
% 
% \end{code}


% 
% 
% \subsection{Tom's example}
% HostA side:
% 
% \begin{code}
% $\newPrin{pAlice}{\{\}};$\\
% $\connect{pc}{\PubK_\bot};$\\
% %\opc{pc}{PubK};\\
% $\outputChan{pc}{\publicKey{pAlice}} ;$\\
% %\Out{\var{pAlice.pubm}}{pc};\\
% $\inputChan{pc}{pkWilly};$\\
% %\In{pKWilly}{pc};\\
% $\newvar{asset}{\Int_{\{pServer,\publicKey{pAlice}\}}}{42};$\\
% $\newvar{WillyGift}{\Int_{\{pServer,\publicKey{pAlice},pkWilly\}}}{12};$\\
% \begin{bl}
% 	$\connectCCert{scS}{\Int_{\{\publicKey{pAlice},pServer\}}}{pServer}{pAlice}$\\
% 	%\occ{pServer}{pAlice}{scS}{\Int}{\{pAlice.pub,pServer\}};\\
% 	$\outputChan{scS}{asset};$
% 	%\Out{asset}{scS};
% \end{bl}
% $|$        
% \begin{bl}
%               $\outputChan{scS}{WillyGift};$
%               %\Out{\var{WillyGift}}{scS};
% \end{bl}              
% \end{code}
%               
%           Host A after reboot.    
%               \begin{code}
% \load{pAlice} ;\\
% \occ{pServer}{pAlice}{scS}{\Int}{\{pAlice.pub,pServer\}};\\
% \In{ServerInfo}{scS};
% \end{code}
% 
% Host B side :
% 
% \begin{code}
%  $\newPrin{pBob}{\{\}};$\\
%  $\connect{pcB}{\PubK_\bot};$\\
%  $\outputChan{pcB}{\publicKey{pBob}};$\\
%  \occ{pBob}{pServer}{c}{\Int}{\{pBob,pServer,pAlice\}};\\
%  \In{received}{c};
% 
% \end{code}

% \subsection{Dropbox example}
% Alice 
% \begin{code}
%  \nwp{pAlice}{\{\}};\\
%  \opc{c}{\MutablePubK};\\
%  \Out{pAlice.mpub}{c};\\
%  \In{pDropbox}{c};\\
%  let pDb = pDropbox in\\
%  \new{int}{\{pAlice.pub,pDb\}}{secret} 345;\\
%   \begin{bl}
% 	\occ{pDb}{pAlice}{cAS}{\Int}{\{pAlice.pub,pDb\}};\\
% 	\Out{secret}{pDb};
%  \end{bl}
%  $|$
%  \begin{bl}
% \In{Bob}{c};\\
% let pBob = Bob in\\
% \new{int}{\{pAlice.pub,pDb,pBob\}}{secretAB} 255;\\
% \occ{pDb}{pAlice}{cAS}{\Int}{\{pAlice.pub,pDb,pBob\}};\\
% \Out{secret}{pDb};
%  \end{bl}
% \end{code}
% 
% % DropBox code without database
% % \begin{code}
% %  \load{Server};\\
% %  \opc{c}{chan(MutablePubk)};\\
% %  \Out{Server;pub}{c};\\
% % %   \comm{All users register (sequentially}}
% %    while(true)
% %    \begin{bl}
% %    \In{user}{c};\\
% %  let pAlice = user in\\
% %  \new{int}{\{Server,pAlice\}}{secretA} 11442;\\
% %   \In{user2}{c};\\
% %  let pBob = user2 in\\
% %  \new{int}{\{Server,pAlice,pBob\}}{secretAB} 3365;\\
% % %   \end{bl}
% % % 
% % % \comm{Later all user send data }
% % %   while(true)
% % %   \begin{bl}
% %  fork
% %  \begin{bl}
% %   \osc{Server}{cSA}{chan(int)}{alpha1};\\
% %   \In{sec}{cSA};\\
% %   if( alpha1 $\lc$ \{Server,pAlice\})
% %   \begin{bl}
% %   secretA=sec;
% %   \end{bl}
% %  \end{bl}
% % 
% % fork
% %  \begin{bl}
% %   \osc{Server}{pAlice}{cSAB}{chan(int)};\\
% %   if( alpha2 < \{Server,pAlice,pBob\})
% %   \begin{bl}
% %   \In{sec}{cSA};\\
% %   secretAB=sec;
% %   \occ{pBob}{Server}{cSB}{Chan(int)}{alpha2};\\
% %   \Out{sec}{cSB};
% %  \end{bl}
% %  \end{bl}
% %   \end{bl}
% %   
% % \end{code}
% 
% Bob code
% \begin{code}
%  \nwp{pBob}{\{\}};\\
%  \opc{c}{\MutablePubK};\\
%  \Out{\var{pBob.mpub}}{c};\\
%  \In{pDropbox}{c};\\
%  \In{pAlice}{c};\\
%  let pDb = pDropbox in\\
%  let pA = pAlice in\\
%  \new{int}{\{Server,pAlice,pBob\}}{secretAB} 0;\\
%  \oscf{pBob}{pDb}{cBS}{\Int}{\{PBob.pub,pDb,pA\}};\\
%  \In{sec}{cSB};\\
%   secretAB=sec;
%  \end{code}
%  
%  \newpage
%  DropBox code with new construct
%  
% \begin{code}
%  \load{Server};\\
%  \nws{int}{$\bot$}{secret1} 0;\\
%  \nws{int}{$\bot$}{secret2} 0;\\
%  \nws{int}{$\bot$}{secret3} 0;\\
%  \nws{int}{$\bot$}{secret4} 0;\\
%  
%  \new{\MutablePubK}{$\bot$}{user1} null;\\
%  \new{\MutablePubK}{$\bot$}{user2} null;\\
%  \new{\MutablePubK}{$\bot$}{user3} null;\\
%  \new{\MutablePubK}{$\bot$}{user4} null;\\
%  
%  \new{\MutablePubK}{$\bot$}{dest1} null;\\
%  \new{\MutablePubK}{$\bot$}{dest2} null;\\
%  \new{\MutablePubK}{$\bot$}{dest3} null;\\
%  \new{\MutablePubK}{$\bot$}{dest4} null;\\
%  
%  
%  \opc{c}{\MutablePubK};\\
%  \Out{\var{Server.mpub}}{c};\\
%  
%    \comm{All users register }\\
%  
%  \new{int}{$\bot$}{i} 1;\\
%  
%  !  \begin{bl}
%    \In{user}{c};\\
%    \In{dest}{c};\\
%   let pAlice = user in\\
%   let pBob = dest in \\
%   if(i = 1)\begin{bl}
%   \set{secret1}{\{Server.pub,pAlice,pBob\}}0;\\
%   user1 = user;
%   dest1 = dest;
%   \end{bl}
% if(i = 2)\begin{bl}
%   \set{secret2}{\{Server.pub,pAlice,pBob\}}0;\\
%   user2 = user;
%   dest2 = dest;             
%   \end{bl}
% if(i = 3)\begin{bl}
%   \set{secret3}{\{Server.pub,pAlice,pBob\}}0;\\
%   user3 = user;
%   dest3 = dest;
%   \end{bl}
% if(i = 4)\begin{bl}
%   \set{secret4}{\{Server.pub,pAlice,pBob\}}0;\\
%   user4 = user;
%   dest4 = dest;
% \end{bl}
%   i = i + 1;
%  \end{bl}
% $|$
%  \begin{bl}
%  let a1 = user1 in \\
%  let b1 = dest1 in \\
% let a2 = user2 in \\
%  let b2 = dest2 in \\
% let a3 = user3 in \\
%  let b3 = dest3 in \\
% let a4 = user4 in \\
%  let b4 = dest4 in \\
%  \end{bl}
%  
%  \end{code}
%  \newpage
%  \begin{code}
% \comm{Later all users send data }\\
% !
% \begin{bl}
% 
%   \osc{Server}{cSAB}{\Int}{alpha};\\
%   \In{sec}{cSA};\\
%   if(alpha = \{Server.pub, a1, b1\})
%   \begin{bl}
% 	\storage{secret1}{sec}{alpha};
%  \end{bl}
%  if(alpha = \{Server.pub, a2, b2\})
%  \begin{bl}
% 	\storage{secret2}{sec}{alpha};
%  \end{bl}
%  \end{bl}
%  
%  \comm{Finally, the server send to each Bob the value}\\
%  $|$!
%  \begin{bl}
%   \occ{b1}{Server}{c1}{\Int}{\{Server.pub,a1,b1\}};\\
%   if(\retrieve{sec}{secret1}{\{Server.pub,a1,b1\}})
%   \begin{bl}
%   \Out{sec}{c1}; 
%   \end{bl}
%     \end{bl}
% $|$!
%  \begin{bl}
%   \occ{b2}{Server}{c2}{\Int}{\{Server.pub,a2,b2\}};\\
%   if(\retrieve{sec}{secret2}{\{Server.pub,a2,b2\}})
%   \begin{bl}
%   \Out{sec}{c2}; 
%   \end{bl}
%     \end{bl}
% 
%   
% \end{code}
% \subsection{Encryption Leaks}
% 
% \begin{code}
%  \new{\Int}{\{Admin\}}{bigSecret} 34;\\
%  \new{\Cipher(int)}{$\bot$}{whatever} \enc{0}{pBob};\\
%  \new{int}{$\bot$}{counter} 0;\\
%  \opc{c}{\Cipher(int)};\\
%  while(counter != 100)\begin{bl}
%                     counter = counter + 1;\\
%                     \Out{whatever}{c};\\
%                    if(bigSecret = counter) \begin{bl}
%                                             whatever=\enc{1}{pBob};\\
%                                            \end{bl}
% 		else
% 			skip;\\
%                     \end{bl}
% 
% \end{code}




% Bob's device
% \begin{code}
%  \new{\Int}{\{pAlice, Bob.\pub\}}{secret} 8;\\
%  \occ{pAlice}{Bob}{c}{\Int}{\{pAlice,Bob.\pub\}};\\
%  if(secret = 8)\begin{bl} 
%                 \Out{secret}{c};
%                \end{bl}
% 
% \end{code}
% 
% Alice's device
% \begin{code}
%  \osc{Alice}{c1}{\Int}{$\alpha$};\\
%  \occ{pElvis}{Alice}{c2}{\Int}{\{Alice.\pub,pElvis\}};\\
%  \In{BobSecret}{c1};\\
%  \Out{1}{c2};\comm{Elvis receives 1 only if secret = 8}\\ 
% \end{code}
% 
% There is a simple fix for that leakage: when we open a channel both sides adds the rights of the channel to the program counter.
% However, this prevent devices to have any less secure channels once they have open a secure one.
% Maybe we should add some kind of Time out command that continues the program in case no input has been received. 
% In that case it can be possible to reset the program-counter.

% \subsection{Leakage example}
% Elvis (untyped)
% \begin{code}
% \new{int}{\{pAlice, pBob\}}{hack} 0 ;\\
% \new{\ProtectType(int)}{\{pAlice,Elvis.\pub\}}{Frack} \protection{hack}{\{pAlice, pBob\}}{\{pAlice,Elvis.\pub\}};\\
% \occ{pAlice}{Elvis}{c}{\ProtectType}{\{pAlice,Elvis.\pub\}};\\
% \Out{Frack}{c};\\
% \In{BobData}{c};
% \end{code}
% 
% Bob (the victim)
% \begin{code}
% \new{int}{\{pAlice, Bob.\pub\}}{leak} 1 ;\\
% \occ{pAlice}{Bob}{c}{\Int}{\{pAlice,Bob.\pub\}};\\
% \Out{leak}{c};
% \end{code}
% 
% Alice (fooled by Elvis)
% \begin{code}
% \osc{Alice}{c1}{\Int}{$\alpha$};\\
% \In{fromBob}{c1};\\
% \osc{Alice}{c2}{\ProtectType(\Int)}{$\beta$};\\
% \In{FromElvis}{c2};\\
% \unpack{\Int}{$\delta$}{ValueofElvis}{FromElvis}{$\alpha$}\begin{bl} 
% \comm{here $\vprin$  $\{ \delta \lc \beta, \alpha \lc \delta\}$}
% 	\new{\ProtectType(int)}{$\beta$}{Frleak} \protection{fromBob}{$\alpha$}{$\beta$}; \comm{because $\vprin\vdash \alpha \lc \beta$}\\
%         \Out{Frleak}{c2}; 
%                       \end{bl}
% 
% 
% \end{code}



% \end{document} 


==> types-syntax.tex <==
%\section{The Language}\label{sec:language}

\section{The Syntax}
\label{sec:syntax}

\subsection{Types}


The most basic values are integers ($\Int$).
We also allow the encryption of any values of type $S$ which has a parametric type ($\Cipher(S)$).
To express confidentiality policy the types of values have a label containing information about which principals
are allowed to learn any information from the value.

Principals mainly consists of a pair of public and secret keys.
The public key is used by labels to identity which principal is allowed to access data and for encryption.
The secret key is used for device to identify themselves for secure connection as well as for decryption:
the knowledge of a secret key means the device has the right to act for this principal.
These values are either created in the device or received by another device,
inside the program these values are referred by names.
This means that the program can receive different keys for a given name depending on the executions.
To still be able to reason about rights statically, 
keys names are not considered as standard types : they cannot be changed with an affectation rule.
% They are stored into memory but can only be used in specific primitive:
% modifying the keys associated to a name is prevented as well as sending keys away through channels
% or encrypting them.
%These limitations avoid putting labels on keys types.
To enable principal to propagate on other devices we use an encapsulation of principal of type $\SecK$.
% These values can be stored as regular variable with a labeled type but these variables cannot be used
% inside rights labels. We detail later the four primitives which are provided to do the conversions 
% between mutable variables and final names used as identities in both direction for both private and public keys.








% Simple types $S$ corresponds to the standard type.
% Here, all types are annotated with rights permissions $R$.
% Rights permissions are set for each principals.
% A principal is an identity which consists in a pair of public and secret key.
% Any device which owns a secret key can claim to be that principal.
% Principals can be created at run time.
% 
% Rights permissions provide two kind of information.
% The first one consists in the of principals who have the right to read the variable.
% The second one expresses who is allowed to get information from the control flow of the variable.
% The syntax for access rights is a pair $R_1 ~ (R_2)$.
% $R_1$ is a set that contains all public key of users that have access to the data and so to the control flow.
% $R_2$ is a set that contains all public key of users that have access only to the control flow.
% Given a right $R = R_1 ~ (R_2)$ we define $R \up = R_1$ the set of people who have full access to the variable
% and $\access{R} = R_1 \cup R_2$ the set of people who have access to the control flow.
% We also denote by $R_1 \lc R_2$ the fact $R_1$ is less confidential than $R_2$ i.e. $R_2 \up \subseteq R_1 \up $ and
% $\access{R_2} \subseteq \access{R_1} $.
% %We allow union and intersection on access rights which are the union and the intersection for both sets ($R \up$ and $R\down$).
% Finally, we can have variables  $\alpha$ that represents some given rights $R$ which has been obtained dynamically.
% 
% Actual data are, here, only of type $\Int$ or secret key. 
% Since we are considering communication between devices, we also have a parametric type $\Chan( S )$ for channels 
% the spread data of type $S$.
% To be able to send data over channel it is possible to encrypt them. Encrypted data have type $\Cipher( S )$.
% Sometime it may be convenient to store the rights access dynamically with the data itself.
% For that, we use $\StoreType( S )$.% and $\FreezeType( S )$ that we will detail later.


Syntax for types appearing into the code are the following.
$S$ represents the standard types. Note that because values might come from untyped attacker
these types play no role to grant confidentiality, they are just for readability reasons.
$R$ is the syntax for label rights. When the program is written $R$ can only be 
a set of public keys whose first key is the public key of a known private key
(just to avoid device to declare variable with unusable types) or a name.
When the program runs, rights are progressively replaced by actual set of public keys.

% The context of typing judgments contains name with general types $T$.
% $T$ can be either a regular type for a variable: $S_R$, a principal type $\PrincipalType$
% or a channel type: $\Chan(S)_R$.
%a final secret key $\PrincipalType$, a final public key $\PubK$, a right $\Rights$,
%a channel type: $\Chan(S)_R$ or a memory cell with mutable rights: $\StoreType(S)$.





\subsection{Principals}

Principals are created with the \cmd{\newPrin{P}{R}} command.
They can by transferred to other devices that owns one of the principals in \KNW.
It consists of a triple of a private key and its corresponding public key as well as the set of allowed owners.
% Principals have type \PrincipalType, this special type is not part of the generic types and do not have a label.
% Therefore, it is impossible to access them but for commands that actually require a Principal.

% A mandatory thing to be able to use a Principal is to act as a principal.
% We made explicit the action of acting as a principal but it is possible to make it transparent
% by considering that owning a principal enable immediately to act as a principal.

To transfer a principal to someone who is allowed to get it, 
a principal has to be released into a regular variable of type \SecK.
The $\RELEASE$ expression encrypts the secret key to provide a transferable variable of type \SecK.
The encryption of the key allows to send it through public channels which is a crucial point.
Indeed, a secret key contains two kinds of information: 
what is the key value that will allow decryption authentication and so on
and the fact the secret key is the one corresponding to a known public key.
When sending a secret key, if the sent key depends on some confidential variable, then a device that will use
that key to authenticate itself would leak information about this confidential variable.
To avoid this issue, we encrypt all private keys such that only the value is protected 
not the fact that a specific key has been released. 
The encryption does not need any parameter: the key is encrypted automatically for all principal that know that key. 

The reverse operation that converts a mutable secret key in a key usable for encryption is $\REGISTER$
which take a secret key and returns, if the decryption succeed, the secret value used as a principal.

\subsection{Rights and public keys}
The language provides several primitives to handle rights and keys.
First, from a principal $P$, it is possible to extract its public key with
$\publicKey{P}$ which provides the key $\pubKeyType$.
%TODO speak about rights?


In addition, since most rights are known only at run-time 
while some commands require one right to be less confidential then another one,
the language provides run-time comparison with the structure $\IF( R_1 \lc R_2 ) C \ELSE C$
which enforce the constraint in the true branch.
%This allows, in the true branch, to store at static time that $ R_1 \lc R_2 $, the set of constraint is stored in $\vprin$.


\subsection{Channels}
In our type system there is three ways to communicate :
\begin{enumerate}
 \item \label{chan:pub} A symmetric public channel which do not require any authentication: $\OPUBCHAN ~c : S; $.  
%  \item \label{chan:unauth} An asymmetric channel, where the server  authenticates himself but not the client.
%  The client side command is $\OUSECCHAN(K_p) ~c : S ;$ and the server side is $\OUSERCHAN(P) ~c : S ; $.
%   \item \label{chan:unauth} An asymmetric channel, where the server  authenticates himself but not the client.
%   However, the client can decide of the rights access of the channel for its side while the server use a virtual right
%   (a right that cannot be packed) for that channel.
%  The client side command is $\OUSECCHAN(K_p) ~c : S \WITH R ;$ and the server side is $\OUSERCHAN(P) ~c : S \DEN \alpha; $.
%  \item \label{chan:anyone}An asymmetric channel, where the server and the client authenticate themselves but the server accept any client.
%   The client side command is \cmd{\OSECCHAN(K_p,P) ~c : S \WITH R;} and the server side is \cmd{\OSECSCHAN(P) ~c : S \DEN \alpha;}.
 \item \label{chan:private} An asymmetric channel, 
 where the server and the client authenticate themselves and the server only accept a designed client.
 The client side is identical to above while the server command is \cmd{\OSECSCHANF(P,K_p) ~c : S \DEN \alpha;}.
\end{enumerate}
Input and output are done with the \cmd{\NEW X = \INPUT( c );} and \cmd{\OUTPUT E \AT c;} commands.

\subsubsection{Encrypting data}
When data are sent over a channel, they may need to be secured: either the channel itself is secure 
or the data are encrypted.
The encryption primitive is the expression $\ENC E \USING R$: it is possible to encrypt for several principals.
To decrypt a data we would like to use a command like $\NEW S X = \DEC E \USING P$. 
However it is not always possible to decrypt because we do not know form the type for who the data is encrypted.
Therefore, we have to deal with dynamic checking. 
This is represented by the full instruction $\IF( \NEW S X = \DEC E \USING P )  C \ELSE C $.

% \subsection{Global storage}
% Regular variables have their rights set once and for all when they are created.
% However sometime it is not possible to know which are the rights at the creation of a variable.
% Consider a server $S$ communicating through two secure channels to a client $A$ and a client $B$.
% $A$ asks the server to send data to $B$



% Sometimes, we trust a principal but we do not want it to access our data (just storing or broadcasting it).
% In that case, it is not useful to encrypt data, we just need to mention that the data should not be read by the principal.
% For that we provide the $\PROTECT E \OF R \WITH R$ expression which is more flexible than encryption since it accepts any right access
% while encryption is limited to one principal for technical reasons.
% In that case, the opening of this construct is $\IF( \NEW S \alpha X = \UNPROTECT E \USING R )  C \ELSE C $,
% where $R$ is the minimal right to allow the opening while the exact rights of $X$ is stored in $\alpha$.
% 
% % As we mention, encryption do not allow to set rights which are not a singleton of principal.
% % Another problem is that it is not possible to store or to send several values which have different rights access without 
% % changing their rights to the higher common denominator.
% % But upgrading the rights of a variable prevent it to be downgraded then.
% % To solve this problem, we provide a $\FREEZE$ primitive.
% % The freezing process store the actual rights with the variable while the pair is set with an higher confidential access rights.
% % Since the value inside the pair cannot be changed while frozen, it is safe to defrost the value anytime without any check.
% % 
% % Note that $\PROTECT$ can be used instead of $\FREEZE$ but $\FREEZE$ avoid the dynamic check.



% Our type system also use a simple version of multi-threading with the $\FORK$ command. 
% This command, which can also be seen as a try catch block, allow a command not to terminate before the
% next command starts. This allows us, to open communication channel and to be sure that the remaining program 
% will still be run even if noone accept the connection.

\subsection{Standard commands}

Finally, we have standard command like conditional branching, declaration of variables and affectation of variables.
We also consider multi-threads devices with the command $|$ and the bang operator to open an arbitrary number of threads.
There is no loop instruction in this language but while loop can be simulated with a bang and the use
of auxiliary variables that allow a new thread to start only when the previous one has ended.

About expressions, we only consider addition of integers but the language can be easily extended to any standard operator.

% We also consider the standard operator $+$ between two integers, the $.\pub$ operator to get the public key of a principal
% and $\{ K_p, \dots, ( K_p , \dots) \}$ to create a new right.

%NOTE: LET used to set the progc to R


% \begin{figure}
%  
% 
% 
% \[
% \begin{array}{rcll}
% C & ::= & \newPrin{P}{R}; ~C &\text{declare a new principal accessible by $R$}
% %\\ & | & \RELEASE P \AS k;  C_1
% \\ & | & \IF(\REGISTER e \AS \Pi \USING P)\THEN C_1 \ELSE C_2 &\text{try to register a secret key as a principal}
% % \\ & | & \IF( \LOAD{P}) C \ELSE C
% % \\ & | & \STORE{P}; C
% %\\ & | & \LET \PubK = X \IN C &\text{provide a copy of a public key which can be used in rights }
% \\ & | & \compare{R}{R} \THEN C \ELSE C &\text{conditional on rights}
% \\
% \\ & | & \connect{c}{S_1,\ldots,S_n}; ~C &\text{connect to an insecure channel}
% \\ & | & \accept{c}{S_1,\ldots,S_n}; ~C &\text{open an insecure channel}
% %\\ & | & \OUSECCHAN(K_p) ~c : S ; C
% %\\ & | & \OUSERCHAN(P) ~c : S ; C
% \\ & | & \connectCCert{c}{R}{{S_1}_{R_1},\ldots,{S_n}_{R_n}}{K_{pub}}{P}; ~C & \text{make a TLS connect to server matching cert additional use client cert} P
% \\ & | & \acceptAny{c}{\alpha}{S_{\alpha_1,\ldots,\alpha_n}}{P}; ~C & \text{accept an TLS connection using cert for any client certificate} P%Because of leakage that may be fixed later
% \\ & | & \acceptCCert{c}{R}{{S_1}_{R_1},\ldots,{S_n}_{R_n}}{P}{K_{pub}}; ~C & \text{ . . `` ``. . for a given client certificate} K_{pub}
% \\ & | & \outputChan{c}{e_1,\ldots,e_n}; ~C &\text{output $e$ on channel $c$}
% \\ & | & \inputChan{c}{x_1,\ldots,x_n}; ~C  &\text{input on channel $c$ and bind to name $x$}
% \\
% \\ & | & \decrypt{P}{e}{x}{S_R} \THEN  C \ELSE C &\text{try to decrypt some data}
% \\
% \\ & | & \paral{C}{C} & \text{parallel composition}
% \\ & | & \bang{C} & \text{replication}
% \\ & | & \newvar{x}{S_R}{e}; ~C & \text{declare a new memory location}
% \\ & | & \assign{x}{e} ; ~C & \text{assignment}
% \\ & | & \assign{x[e]}{e} ; ~C & \text{assignment}
% \\ & | & \cond{e}{e} \THEN  C \ELSE C & \text{conditional}
% %\\ & | & \WHILE (E = 0) \{ C \} C
% \\ & | & \SKIP
% \end{array}
% \]
% \caption{The commands syntax
% %Here $\alpha$ stands for fresh variable of type $\Rights$, $X$ for a fresh variable neither of type right or principal.
% }\label{fig:syntax-commands}
% \end{figure}
% \begin{figure}
% \[
%  \begin{array}{rcll}
% e & ::= & X & \text{the contents of a memory location}
% \\ & | & 0,1,2,\dots & \text{an integer}
% \\ & | & e_1 + e_2 & \text{a sum}
% \\ & | & P.\pubm & \text{the value of the public key of a principal}
% \\ & | & \RELEASE P & \text{an encapsulation of the private key of a principal}
% \\ & | & \encrypt{R}{n}{e}~~~~& \text{a cipher containing $e$ encrypted for principals in $R$ and nonce $n$}
% %\\ & | & \PROTECT E \OF R \WITH R
% %\\ & | & \{ K_p, \dots \}
% \end{array}
% \]
% \caption{Syntax for expressions}\label{fig:syntax-expr}
% \end{figure}







